Translating Recursive Probabilistic Programs to Factor Graph Grammars

It is natural for probabilistic programs to use conditionals to express alternative substructures in models, and loops (recursion) to express repeated substructures in models. Thus, probabilistic programs with conditionals and recursion motivate ongoing interest in efficient and general inference. A factor graph grammar (FGG) generates a set of factor graphs that do not all need to be enumerated in order to perform inference. We provide a semantics-preserving translation from first-order probabilistic programs with conditionals and recursion to FGGs.

==> examples/hmm.tex <==
\begin{align*}
% minimize |y(e)-y(v1)|
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[fac](e) at (0,-0.0) {$S$};
\node[ext,right of=e](v1) {$v_{1}$};
\draw (e) edge[out=0,in=180] (v1);
\end{tikzpicture}
&\longrightarrow
% minimize |y(e2)-y(v2)|
% minimize |y(v2)-y(e1)|
% minimize |y(e1)-y(v1)|
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[fac,label=below:{$v_{2}=BOS$}](e2) at (0,-0.0) {};
\node[var,right of=e2](v2) {$v_{2}$};
\node[fac,right of=v2](e1) {$step$};
\node[ext,right of=e1](v1) {$v_{1}$};
\draw (e2) edge[out=0,in=180] (v2);
\draw (v2) edge[out=0,in=180] (e1);
\draw (e1) edge[out=0,in=180] (v1);
\end{tikzpicture}
\\
% minimize |y(e7)-y(v7)|
% minimize |y(q)-y(e7)|
% minimize |y(v4)-y(e7)|
% y(q)-y(v4) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,0.5) {$q$};
\node[ext](v4) at (0,-0.5) {$r$};
\node[fac](e7) at (1,-0.0) {$e_{7}$};
\node[ext,right of=e7](v7) {$v_{10}$};
\draw (e7) edge[out=0,in=180] (v7);
\draw (q) edge[out=0,in=180] (e7);
\draw (v4) edge[out=0,in=180] (e7);
\end{tikzpicture}
&\longrightarrow
% minimize |y(v4)-y(e8)|
% minimize |y(e8)-y(v8)|
% minimize |y(v8)-y(v7_t)|
% minimize |y(e10)-y(v10)|
% y(q)-y(v4) ≥ 1
% y(e8)-y(e10) ≥ 1
% y(v8)-y(v10) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,1.0) {$q$};
\node[ext](v4) at (0,-0.0) {$r$};
\node[fac,label=below:{$v_{8}=r=EOS$},right of=v4](e8) {};
\node[fac,label=below:{$v_{10}=unit$}](e10) at (1,-1.0) {};
\node[var,right of=e8](v8) {$v_{8}$};
\node[ext,right of=e10](v10) {$v_{10}$};
\node[fac,label=below:{$v_{8}=\textbf{true}$},right of=v8](v7_t) {};
\draw (v4) edge[out=0,in=180] (e8);
\draw (e8) edge[out=0,in=180] (v8);
\draw (v8) edge[out=0,in=180] (v7_t);
\draw (e10) edge[out=0,in=180] (v10);
\end{tikzpicture}
\\
% minimize |y(e7)-y(v7)|
% minimize |y(q)-y(e7)|
% minimize |y(v4)-y(e7)|
% y(q)-y(v4) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,0.5) {$q$};
\node[ext](v4) at (0,-0.5) {$r$};
\node[fac](e7) at (1,-0.0) {$e_{7}$};
\node[ext,right of=e7](v7) {$v_{15}$};
\draw (e7) edge[out=0,in=180] (v7);
\draw (q) edge[out=0,in=180] (e7);
\draw (v4) edge[out=0,in=180] (e7);
\end{tikzpicture}
&\longrightarrow
% minimize |y(v4)-y(e8)|
% minimize |y(e8)-y(v8)|
% minimize |y(v8)-y(v7_f)|
% minimize |y(q)-y(e13)|
% minimize |y(e13)-y(v13)|
% minimize |y(v13)-y(e12)|
% minimize |y(e12)-y(v12)|
% minimize |y(v4)-y(e15)|
% minimize |y(e15)-y(v15)|
% y(q)-y(v4) ≥ 1
% y(e8)-y(e13) ≥ 1
% y(v8)-y(v13) ≥ 1
% y(v7_f)-y(e12) ≥ 1
% y(e13)-y(e15) ≥ 1
% y(v13)-y(v15) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,0.0) {$q$};
\node[ext](v4) at (0,-1.0) {$r$};
\node[fac,label=below:{$v_{8}=r=EOS$}](e8) at (1,1.0) {};
\node[fac,label=below:{$v_{13}=e(q)$},right of=q](e13) {};
\node[fac,right of=v4](e15) {$step$};
\node[var,right of=e8](v8) {$v_{8}$};
\node[var,right of=e13](v13) {$v_{13}$};
\node[ext,right of=e15](v15) {$v_{15}$};
\node[fac,label=below:{$v_{8}=\textbf{false}$},right of=v8](v7_f) {};
\node[fac,label=below:{$v_{13}(v_{12})$},right of=v13](e12) {};
\node[var,right of=e12](v12) {$w$};
\draw (v4) edge[out=0,in=180] (e8);
\draw (e8) edge[out=0,in=180] (v8);
\draw (v8) edge[out=0,in=180] (v7_f);
\draw (q) edge[out=0,in=180] (e13);
\draw (e13) edge[out=0,in=180] (v13);
\draw (v13) edge[out=0,in=180] (e12);
\draw (e12) edge[out=0,in=180] (v12);
\draw (v4) edge[out=0,in=180] (e15);
\draw (e15) edge[out=0,in=180] (v15);
\end{tikzpicture}
\\
% minimize |y(q)-y(e)|
% minimize |y(e)-y(v7)|
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,-0.0) {$q$};
\node[fac,right of=q](e) {$step$};
\node[ext,right of=e](v7) {$v_{7}$};
\draw (q) edge[out=0,in=180] (e);
\draw (e) edge[out=0,in=180] (v7);
\end{tikzpicture}
&\longrightarrow
% minimize |y(q)-y(e5)|
% minimize |y(e5)-y(v5)|
% minimize |y(v5)-y(e4)|
% minimize |y(e4)-y(v4)|
% minimize |y(v4)-y(e7)|
% minimize |y(e7)-y(v7)|
% minimize |y(q)-y(virtual_7)|
% minimize |y(virtual_7)-y(virtual_8)|
% minimize |y(virtual_8)-y(virtual_9)|
% minimize |y(virtual_9)-y(virtual_10)|
% minimize |y(virtual_10)-y(e7)|
% y(e5)-y(virtual_7) ≥ 1
% y(v5)-y(virtual_8) ≥ 1
% y(e4)-y(virtual_9) ≥ 1
% y(v4)-y(virtual_10) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,-0.0) {$q$};
\node[fac,label=below:{$v_{5}=t(q)$}](e5) at (1,0.5) {};
\node[coordinate](virtual_7) at (1,-0.5) {$$};
\node[var,right of=e5](v5) {$v_{5}$};
\node[coordinate,right of=virtual_7](virtual_8) {$$};
\node[fac,label=below:{$v_{5}(v_{4})$},right of=v5](e4) {};
\node[coordinate,right of=virtual_8](virtual_9) {$$};
\node[var,right of=e4](v4) {$r$};
\node[coordinate,right of=virtual_9](virtual_10) {$$};
\node[fac](e7) at (5,-0.0) {$e_{7}$};
\node[ext,right of=e7](v7) {$v_{7}$};
\draw (q) edge[out=0,in=180] (e5);
\draw (e5) edge[out=0,in=180] (v5);
\draw (v5) edge[out=0,in=180] (e4);
\draw (e4) edge[out=0,in=180] (v4);
\draw (v4) edge[out=0,in=180] (e7);
\draw (e7) edge[out=0,in=180] (v7);
\draw (q) edge[out=0,in=180] (virtual_7);
\draw (virtual_7) edge[out=0,in=180] (virtual_8);
\draw (virtual_8) edge[out=0,in=180] (virtual_9);
\draw (virtual_9) edge[out=0,in=180] (virtual_10);
\draw (virtual_10) edge[out=0,in=180] (e7);
\end{tikzpicture}
\end{align*}


==> examples/hmmw.tex <==
\begin{align*}
% minimize |y(e)-y(v1)|
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[fac](e) at (0,-0.0) {$S$};
\node[ext,right of=e](v1) {$v_{1}$};
\draw (e) edge[out=0,in=180] (v1);
\end{tikzpicture}
&\longrightarrow
% minimize |y(e2)-y(v2)|
% minimize |y(v2)-y(e1)|
% minimize |y(e1)-y(v1)|
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[fac,label=below:{$v_{2}=BOS$}](e2) at (0,-0.0) {};
\node[var,right of=e2](v2) {$v_{2}$};
\node[fac,right of=v2](e1) {$step$};
\node[ext,right of=e1](v1) {$v_{1}$};
\draw (e2) edge[out=0,in=180] (v2);
\draw (v2) edge[out=0,in=180] (e1);
\draw (e1) edge[out=0,in=180] (v1);
\end{tikzpicture}
\\
% minimize |y(e7)-y(v7)|
% minimize |y(q)-y(e7)|
% minimize |y(w)-y(e7)|
% minimize |y(v4)-y(e7)|
% y(q)-y(w) ≥ 1
% y(w)-y(v4) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,1.0) {$q$};
\node[ext](w) at (0,-0.0) {$w$};
\node[ext](v4) at (0,-1.0) {$r$};
\node[fac](e7) at (1,-0.0) {$e_{7}$};
\node[ext,right of=e7](v7) {$v_{13}$};
\draw (e7) edge[out=0,in=180] (v7);
\draw (q) edge[out=0,in=180] (e7);
\draw (w) edge[out=0,in=180] (e7);
\draw (v4) edge[out=0,in=180] (e7);
\end{tikzpicture}
&\longrightarrow
% minimize |y(v4)-y(e8)|
% minimize |y(e8)-y(v8)|
% minimize |y(v8)-y(v7_t)|
% minimize |y(w)-y(e11)|
% minimize |y(e11)-y(v11)|
% minimize |y(v11)-y(v10_t)|
% minimize |y(e13)-y(v13)|
% y(q)-y(w) ≥ 1
% y(w)-y(v4) ≥ 1
% y(e8)-y(e11) ≥ 1
% y(v8)-y(v11) ≥ 1
% y(v7_t)-y(v10_t) ≥ 1
% y(e11)-y(e13) ≥ 1
% y(v11)-y(v13) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,1.0) {$q$};
\node[ext](w) at (0,-0.0) {$w$};
\node[ext](v4) at (0,-1.0) {$r$};
\node[fac,label=below:{$v_{8}=r=EOS$}](e8) at (1,1.0) {};
\node[fac,label=below:{$v_{11}=w=nil$},right of=w](e11) {};
\node[fac,label=below:{$v_{13}=unit$}](e13) at (1,-1.0) {};
\node[var,right of=e8](v8) {$v_{8}$};
\node[var,right of=e11](v11) {$v_{11}$};
\node[ext,right of=e13](v13) {$v_{13}$};
\node[fac,label=below:{$v_{8}=\textbf{true}$},right of=v8](v7_t) {};
\node[fac,label=below:{$v_{11}=\textbf{true}$},right of=v11](v10_t) {};
\draw (v4) edge[out=0,in=180] (e8);
\draw (e8) edge[out=0,in=180] (v8);
\draw (v8) edge[out=0,in=180] (v7_t);
\draw (w) edge[out=0,in=180] (e11);
\draw (e11) edge[out=0,in=180] (v11);
\draw (v11) edge[out=0,in=180] (v10_t);
\draw (e13) edge[out=0,in=180] (v13);
\end{tikzpicture}
\\
% minimize |y(e7)-y(v7)|
% minimize |y(q)-y(e7)|
% minimize |y(w)-y(e7)|
% minimize |y(v4)-y(e7)|
% y(q)-y(w) ≥ 1
% y(w)-y(v4) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,1.0) {$q$};
\node[ext](w) at (0,-0.0) {$w$};
\node[ext](v4) at (0,-1.0) {$r$};
\node[fac](e7) at (1,-0.0) {$e_{7}$};
\node[ext,right of=e7](v7) {$v_{23}$};
\draw (e7) edge[out=0,in=180] (v7);
\draw (q) edge[out=0,in=180] (e7);
\draw (w) edge[out=0,in=180] (e7);
\draw (v4) edge[out=0,in=180] (e7);
\end{tikzpicture}
&\longrightarrow
% minimize |y(v4)-y(e8)|
% minimize |y(e8)-y(v8)|
% minimize |y(v8)-y(v7_f)|
% minimize |y(q)-y(e17)|
% minimize |y(e17)-y(v17)|
% minimize |y(v17)-y(e16)|
% minimize |y(e16)-y(v16)|
% minimize |y(v16)-y(e20)|
% minimize |y(e20)-y(v20)|
% minimize |y(v20)-y(v19_t)|
% minimize |y(w)-y(e25)|
% minimize |y(e25)-y(v25)|
% minimize |y(v25)-y(e23)|
% minimize |y(e23)-y(v23)|
% minimize |y(w)-y(virtual_17)|
% minimize |y(virtual_17)-y(virtual_18)|
% minimize |y(virtual_18)-y(virtual_19)|
% minimize |y(virtual_19)-y(virtual_20)|
% minimize |y(virtual_20)-y(e20)|
% minimize |y(v4)-y(virtual_21)|
% minimize |y(virtual_21)-y(virtual_22)|
% minimize |y(virtual_22)-y(e23)|
% y(q)-y(w) ≥ 1
% y(w)-y(v4) ≥ 1
% y(e8)-y(e17) ≥ 1
% y(v8)-y(v17) ≥ 1
% y(v7_f)-y(e16) ≥ 1
% y(e17)-y(e25) ≥ 1
% y(v17)-y(v25) ≥ 1
% y(e16)-y(e23) ≥ 1
% y(v16)-y(v23) ≥ 1
% y(e25)-y(virtual_17) ≥ 1
% y(v25)-y(virtual_18) ≥ 1
% y(e23)-y(virtual_19) ≥ 1
% y(v23)-y(virtual_20) ≥ 1
% y(virtual_17)-y(virtual_21) ≥ 1
% y(virtual_18)-y(virtual_22) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,1.0) {$q$};
\node[ext](w) at (0,-0.5) {$w$};
\node[ext](v4) at (0,-2.0) {$r$};
\node[fac,label=below:{$v_{8}=r=EOS$}](e8) at (1,2.0) {};
\node[fac,label=below:{$v_{17}=e(q)$},right of=q](e17) {};
\node[fac,label=below:{$v_{25}=cdr(w)$}](e25) at (1,-0.0) {};
\node[coordinate](virtual_17) at (1,-1.0) {$$};
\node[coordinate,right of=v4](virtual_21) {$$};
\node[var,right of=e8](v8) {$v_{8}$};
\node[var,right of=e17](v17) {$v_{17}$};
\node[var,right of=e25](v25) {$v_{25}$};
\node[coordinate,right of=virtual_17](virtual_18) {$$};
\node[coordinate,right of=virtual_21](virtual_22) {$$};
\node[fac,label=below:{$v_{8}=\textbf{false}$},right of=v8](v7_f) {};
\node[fac,label=below:{$v_{17}(v_{16})$},right of=v17](e16) {};
\node[fac](e23) at (3,-0.0) {$step$};
\node[coordinate,right of=virtual_18](virtual_19) {$$};
\node[var,right of=e16](v16) {$w1$};
\node[ext,right of=e23](v23) {$v_{23}$};
\node[coordinate,right of=virtual_19](virtual_20) {$$};
\node[fac,label=below:{$v_{20}=w1=w1$}](e20) at (5,0.0) {};
\node[var,right of=e20](v20) {$v_{20}$};
\node[fac,label=below:{$v_{20}=\textbf{true}$},right of=v20](v19_t) {};
\draw (v4) edge[out=0,in=180] (e8);
\draw (e8) edge[out=0,in=180] (v8);
\draw (v8) edge[out=0,in=180] (v7_f);
\draw (q) edge[out=0,in=180] (e17);
\draw (e17) edge[out=0,in=180] (v17);
\draw (v17) edge[out=0,in=180] (e16);
\draw (e16) edge[out=0,in=180] (v16);
\draw (v16) edge[out=0,in=180] (e20);
\draw (e20) edge[out=0,in=180] (v20);
\draw (v20) edge[out=0,in=180] (v19_t);
\draw (w) edge[out=0,in=180] (e25);
\draw (e25) edge[out=0,in=180] (v25);
\draw (v25) edge[out=0,in=180] (e23);
\draw (e23) edge[out=0,in=180] (v23);
\draw (w) edge[out=0,in=180] (virtual_17);
\draw (virtual_17) edge[out=0,in=180] (virtual_18);
\draw (virtual_18) edge[out=0,in=180] (virtual_19);
\draw (virtual_19) edge[out=0,in=180] (virtual_20);
\draw (virtual_20) edge[out=0,in=180] (e20);
\draw (v4) edge[out=0,in=180] (virtual_21);
\draw (virtual_21) edge[out=0,in=180] (virtual_22);
\draw (virtual_22) edge[out=0,in=180] (e23);
\end{tikzpicture}
\\
% minimize |y(q)-y(e)|
% minimize |y(w)-y(e)|
% minimize |y(e)-y(v7)|
% y(q)-y(w) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,0.5) {$q$};
\node[ext](w) at (0,-0.5) {$w$};
\node[fac](e) at (1,-0.0) {$step$};
\node[ext,right of=e](v7) {$v_{7}$};
\draw (q) edge[out=0,in=180] (e);
\draw (w) edge[out=0,in=180] (e);
\draw (e) edge[out=0,in=180] (v7);
\end{tikzpicture}
&\longrightarrow
% minimize |y(q)-y(e5)|
% minimize |y(e5)-y(v5)|
% minimize |y(v5)-y(e4)|
% minimize |y(e4)-y(v4)|
% minimize |y(v4)-y(e7)|
% minimize |y(e7)-y(v7)|
% minimize |y(q)-y(virtual_8)|
% minimize |y(virtual_8)-y(virtual_9)|
% minimize |y(virtual_9)-y(virtual_10)|
% minimize |y(virtual_10)-y(virtual_11)|
% minimize |y(virtual_11)-y(e7)|
% minimize |y(w)-y(virtual_12)|
% minimize |y(virtual_12)-y(virtual_13)|
% minimize |y(virtual_13)-y(virtual_14)|
% minimize |y(virtual_14)-y(virtual_15)|
% minimize |y(virtual_15)-y(e7)|
% y(q)-y(w) ≥ 1
% y(e5)-y(virtual_8) ≥ 1
% y(v5)-y(virtual_9) ≥ 1
% y(e4)-y(virtual_10) ≥ 1
% y(v4)-y(virtual_11) ≥ 1
% y(virtual_8)-y(virtual_12) ≥ 1
% y(virtual_9)-y(virtual_13) ≥ 1
% y(virtual_10)-y(virtual_14) ≥ 1
% y(virtual_11)-y(virtual_15) ≥ 1
\begin{tikzpicture}[node distance=1cm,x=1cm]
\node[ext](q) at (0,0.5) {$q$};
\node[ext](w) at (0,-1.0) {$w$};
\node[fac,label=below:{$v_{5}=t(q)$}](e5) at (1,1.0) {};
\node[coordinate](virtual_8) at (1,-0.0) {$$};
\node[coordinate,right of=w](virtual_12) {$$};
\node[var,right of=e5](v5) {$v_{5}$};
\node[coordinate,right of=virtual_8](virtual_9) {$$};
\node[coordinate,right of=virtual_12](virtual_13) {$$};
\node[fac,label=below:{$v_{5}(v_{4})$},right of=v5](e4) {};
\node[coordinate,right of=virtual_9](virtual_10) {$$};
\node[coordinate,right of=virtual_13](virtual_14) {$$};
\node[var,right of=e4](v4) {$r$};
\node[coordinate,right of=virtual_10](virtual_11) {$$};
\node[coordinate,right of=virtual_14](virtual_15) {$$};
\node[fac](e7) at (5,-0.0) {$e_{7}$};
\node[ext,right of=e7](v7) {$v_{7}$};
\draw (q) edge[out=0,in=180] (e5);
\draw (e5) edge[out=0,in=180] (v5);
\draw (v5) edge[out=0,in=180] (e4);
\draw (e4) edge[out=0,in=180] (v4);
\draw (v4) edge[out=0,in=180] (e7);
\draw (e7) edge[out=0,in=180] (v7);
\draw (q) edge[out=0,in=180] (virtual_8);
\draw (virtual_8) edge[out=0,in=180] (virtual_9);
\draw (virtual_9) edge[out=0,in=180] (virtual_10);
\draw (virtual_10) edge[out=0,in=180] (virtual_11);
\draw (virtual_11) edge[out=0,in=180] (e7);
\draw (w) edge[out=0,in=180] (virtual_12);
\draw (virtual_12) edge[out=0,in=180] (virtual_13);
\draw (virtual_13) edge[out=0,in=180] (virtual_14);
\draw (virtual_14) edge[out=0,in=180] (virtual_15);
\draw (virtual_15) edge[out=0,in=180] (e7);
\end{tikzpicture}
\end{align*}

